Are All Good Word Vector Spaces Isomorphic?

Existing algorithms for aligning cross-lingual word vector spaces assume that vector spaces are approximately isomorphic. As a result, they perform poorly or fail completely on non-isomorphic spaces. Such non-isomorphism has been hypothesised to result from typological differences between languages. In this work, we ask whether non-isomorphism is also crucially a sign of degenerate word vector spaces. We present a series of experiments across diverse languages which show that variance in performance across language pairs is not only due to typological differences, but can mostly be attributed to the size of the monolingual resources available, and to the properties and duration of monolingual training (e.g. "under-training").

==> 04-infb.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{0.318\linewidth}
        \centering
        \includegraphics[width=0.98\linewidth]{images/long-training_hfreq.pdf}
        %\vspace{-0.7em}
        \caption{\hf subset (\es)}
        \label{fig:iso-es-hfreq}
    \end{subfigure}
    \begin{subfigure}[t]{0.318\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{images/long-training_mfreq.pdf}
        %\vspace{-0.7em}
        \caption{\mf subset (\es)}
        \label{fig:iso-es-mfreq}
    \end{subfigure}
        \begin{subfigure}[t]{0.318\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{images/long-training_lfreq.pdf}
        %\vspace{-0.7em}
        \caption{\lf subset (\es)}
        \label{fig:iso-es-lfreq}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Monolingual learning dynamics and isomorphism (RSIM): We align a partially trained \textsc{es} vector space, after seeing $M$ word tokens, with a fully trained \textsc{en} vector space, and evaluate on (a) \hf, (b) \mf, and (c) \lf test sets. While BDI performance plateaus, RSIM does not.}
    \vspace{-1.5mm}
\label{fig:IB}
\end{figure*}

In our experiments, we have measured how training monolingual word embeddings improves their isomorphism with word embeddings in other languages. In doing so, we made an interesting observation: {\em Isomorphism increases even beyond the point in the training process where validation (BLI) scores and training losses plateau.} To see this, consider Figure~\ref{fig:IB}. One possible explanation for this may be that isomorphism increases as learning dynamics drive us into high-entropy solutions. Recent studies of learning dynamics in deep neural nets observe that flatter optima generalize better than sharp optima \cite{Zhang:ea:18}: intuitively, it is because sharp minima correspond to more
complex, likely over-fitted, models. \newcite{Zhang:ea:18} show that analogous to the energy-entropy competition in statistical physics, wide but shallow minima can be optimal if the system is undersampled. %In the high dimensional limit, wide minima are preferable over narrow ones even at the expense of higher error in-sample; and the extent to which wide minima are preferable is dependent on the degree of undersampling and approximation noise.
SGD is assumed to generalize well because its inherent anisotropic noise biases it towards higher entropy minima. We hypothesize a similar explanation of our observations in terms of energy-entropy competition. Once loss is minimized, the random oscillations due to SGD noise lead the weights toward a high-entropy solution. We hypothesize monolingual high-entropy minima are more likely to be isomorphic. A related possible explanation is that the increased isomorphism results from model compression. This is analogous to the idea of two-phase learning \cite{shwartz2017opening}, whereby the initial fast convergence of SGD
is related to sufficiency of the representation, while the later asymptotic phase is related
to compression of the activations. 
